Precision determination of the strong coupling constant within a global PDF analysis

We present a determination of the strong coupling constant $\alpha_s(m_Z)$ based on the NNPDF3.1 determination of parton distributions, which for the first time includes constraints from jet production, top-quark pair differential distributions, and the $Z$ $p_T$ distributions using exact NNLO theory. Our result is based on a novel extension of the NNPDF methodology - the correlated replica method - which allows for a simultaneous determination of $\alpha_s$ and the PDFs with all correlations between them fully taken into account. We study in detail all relevant sources of experimental, methodological and theoretical uncertainty. At NNLO we find $\alpha_s(m_Z) = 0.1185 \pm 0.0005^\text{(exp)}\pm 0.0001^\text{(meth)}$, showing that methodological uncertainties are negligible. We conservatively estimate the theoretical uncertainty due to missing higher order QCD corrections (N$^3$LO and beyond) from half the shift between the NLO and NNLO $\alpha_s$ values, finding $\Delta\alpha^{\rm th}_s =0.0011$.

==> pull_table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[tp]
\begin{center}
  \footnotesize
      \renewcommand{\arraystretch}{1.18}
\begin{tabular}{l|c|c|c}

  &  Pull & $\as^{(\min\chi^2_p)}$ &   $\sigma_\alpha^{(0),p}$ \\
\toprule
NMC    &  0.02     &0.1192  &0.0048        \\    
SLAC    &  0.20     & 0.1205  &	   0.0023     \\    
BCDMS    &   -0.10   &  0.1176   & 0.0020       \\    
CHORUS  $\nu$ CC  &  -0.02   &  0.1115  &  0.0140     \\    
CHORUS  $\bar{\nu}$ CC  & -0.00    & 0.1178   &   0.0235    \\    
NuTeV dimuon  $\nu$ CC  &-0.01  &   0.1060    &  0.0283     \\    
NuTeV dimuon  $\bar{\nu}$ CC  & -0.00 &   0.1117      &  0.0287     \\    
\midrule
HERA I+II incl   &   0.10  &  0.1191   &   0.0017     \\      
HERA $F_2^c$    &  -0.02 &    0.1130    &  0.0129     \\    
HERA $F_2^b$    & 0.03   & 0.1397     &  0.0205   \\    
\midrule
DY E866 $\sigma^d_{\rm DY}/\sigma^p_{\rm DY}$ &  0.00    &  0.1174 &  0.0728       \\    
DY E886 $\sigma^p$    &-0.00      &  0.0784 & 0.1615      \\    
DY E605  $\sigma^p$   &  0.00   &   0.1197 &  0.0278    \\    
CDF $Z$ rap    & 0.00  & 0.2031      &  1.409      \\    
D0 $Z$ rap    &   0.00  &  0.1105   &     0.1462  \\    
D0 $W\to e\nu$  asy   &   0.00    &0.0788   &   0.0886    \\    
D0 $W\to \mu\nu$  asy      &     0.00 & 0.1166 & 0.0231      \\    
\midrule
ATLAS total   &  {\bf 1.29 }  &   {\bf 0.1208  }      &   {\bf 0.0010  }    \\    
ATLAS $W,Z$ 7 TeV 2010    & -0.01   & 0.1181    &  0.0057      \\    
ATLAS high-mass DY 7 TeV    & 0.00  & 0.1110    &   0.1235    \\    
ATLAS low-mass DY 2011    &  -0.10    & 0.1153   &  0.0041      \\    
ATLAS $W,Z$ 7 TeV 2011    &0.04      & 0.1208  &  0.0055      \\    
ATLAS jets 2011 7 TeV     & 0.28  &   0.1230   &0.0029      \\    
ATLAS $Z$ $p_T$ 8 TeV $(p_T^{ll},M_{ll})$       &  0.73 & 0.1230 &0.0018      \\    
ATLAS $Z$ $p_T$ 8 TeV $(p_T^{ll},y_{ll})$    &   0.41 &  0.1248    & 0.0028     \\    
ATLAS $\sigma_{tt}^{\rm tot}$     &  0.20   &  0.1197   &0.0018       \\    
ATLAS $t\bar{t}$ rap    &   -0.07   & 0.1108  &   0.0073     \\
\midrule
CMS total   &   {\bf 1.47}  & {\bf 0.1223  }    &   {\bf 0.0012 }   \\    
CMS $W$ asy 840 pb     &  0.00  &  0.1080   &  0.0586    \\    
CMS $W$ asy 4.7 fb     &   0.00   & 0.1167  &  0.0454     \\    
CMS Drell-Yan 2D 2011    & 0.50   &0.1284     &0.0032       \\    
CMS $W$ rap 8 TeV    &   -0.02 &    0.1173  &  0.0060   \\    
CMS jets 7 TeV 2011     & 0.08   & 0.1207     & 0.0037      \\    
CMS $Z$ $p_T$ 8 TeV $(p_T^{ll},M_{ll})$    & 0.74   &0.1242    &  0.0020    \\    
CMS $\sigma_{tt}^{\rm tot}$     &  -0.03   & 0.1183    & 0.0017       \\    
CMS $t\bar{t}$ rap    &0.00   &  0.1176   &  0.0236   \\
\midrule
LHCb total   & {\bf 0.07}	&  {\bf0.1192  }      &   {\bf 0.0023 }    \\
LHCb $Z$ 940 pb   & 0.03 &    0.1234      & 0.0095       \\    
LHCb $Z\to ee$ 2 fb    & 0.05 &     0.1194   &     0.0033  \\    
LHCb $W,Z \to \mu$ 7 TeV    & 0.00&    0.1227      &0.0329       \\    
LHCb $W,Z \to \mu$ 8 TeV    & -0.08    &  0.1166  &  0.0036      \\    
\midrule
Collider DIS  & 0.45 & 0.1200  &  0.0013\\
Jets 	& 	0.03 & 0.1213	& 0.0068 \\
$Z p_T$ 	&	1.79	 &0.1241 &0.0013 \\
FT neutrino DIS	 &	-0.01 & 0.1110	& 0.0220 \\
FT lepton DIS	&0.06	&0.1186	&0.0011 \\
LHC DY	 &1.01	& 0.1213	&0.0012 \\
FT DY	&0.00	&0.0900	&0.1280 \\
Top 	&	-0.04 &0.1184	&0.0011\\
\midrule
{\bf Total}    & {\bf -} & {\bf 0.11845  }      & {\bf 0.00052 }   \\    
\bottomrule
\end{tabular}
\vspace{0.3cm}
\caption{\small
  \label{table:nnlo_global_pulls}
  The pulls $P_p$, Eq.~(\ref{eq:pulldef}), for the individual
  experiments included in the NNLO fit, together
  with  the preferred $\as^{(0),p}$ values
  and the corresponding uncertainty
  $\sigma_\alpha^{(0),p}$ in each case.
}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

